Intersections of Web3 and AI -- View in 2024

This paper summarises the intersection of Web3 and AI technologies, synergies between these technologies, and gaps that we suggest exist in the conception of the possible integrations of these technologies. The summary is informed by a comprehensive literature review of current academic and industry papers, analyst reports, and Ethereum research community blogposts. We focus our contribution on the perceived gaps and detail some novel approaches that would benefit the blockchain/Web3 ecosystem. We believe that the overview presented in this paper will help guide researchers interested in the intersection of Web3 and AI technologies.

==> modelcollapse.tex <==
% -------------------------------------
\subsection{Model Collapse}
% -------------------------------------
\label{sec:modelcollapse}

\glspl*{llm} are trained on many public data sources as described in Section \ref{sec:litrevphilosophical}, \nameref{sec:litrevphilosophical}, \ref{sec:litrevfuture} \nameref{sec:litrevfuture}. Since many users are using \glspl*{llm} to generate content that is being put onto those same public fora, future versions of those \glspl*{llm} are very likely to ingest content generated by earlier versions of themselves. It is not difficult to envision a future in which \glspl*{llm} become trained on an ever-increasing amount of machine-generated content and a decreasing amount of human-generated content. The ramifications are intriguing; without a change in the way the models are trained their weights will be increasingly influenced by machine-generated content. Human-generated content could even become a minority input for some models.

The unintended or unrecognised prevalence of machine-generated content in training data coupled with the failure of \glspl*{llm} to differentiate human- and machine-generated content is known as model collapse \cite{Shumailov_Shumaylov_Zhao_Gal_Papernot_Anderson_2024}. An \gls*{llm} in model collapse would not treat human-generated content in a preferred manner. Instead, a positive feedback loop would be set up whereby new \glspl*{llm} will learn to write like old \glspl*{llm}.

Possible mitigations for model collapse include the use of data provenance techniques to label human- and/or machine-generated content  \cite{baioumy_ai_2024}. Such approaches are limited to mitigating, not solving, the problem of model collapse because many systems and users will simply choose to ignore data provenance hint publication.

Other mitigations may be possible via governmental \gls*{ai} strategies and subsequent regulation \cite{tjondronegoro_strategic_2024}. A common analysis technique for such frameworks is the PESTEL analysis technique. PESTEL is an acronym standing for political, economic, social, technological, environmental, and legal factors in an environment external to an organisation \cite{aguilar1967scanning}. Tjondronegoro notes that a PESTEL analysis of AI adoption barriers and themes suggests that ``Data availability, quality, and structure'' fall under the technology rubric. Governments may choose to selectively regulate some data availability to reduce some negative consequences of model collapse.

None of the currently-identified mitigations to model collapse appear to be sufficient to prevent the phenomenon from occurring. More research into this area is urgently needed.


==> scholargpt.tex <==
% ----------------------------------------
\subsubsection{Experiences with ScholarGPT}
% ----------------------------------------
\label{scholargpt}

We attempted to construct a literature review in partnership with OpenAI's ScholarGPT and its integrations with ScholarAI and sider.ai. This work was performed in May and June 2024 using the ScholarGPT based upon ChatGPT 4. It was created as an experiment in using those tools to accelerate the review and analysis of existing scholarly works. Generated outputs were carefully checked and edited for correctness and validity. Significant hallucinations were detected by ScholarGPT during review and were removed. The end result did not compare favourably to a literature review created using traditional means.

ScholarGPT was useful in conducting a bibliographic analysis of research papers that we had identified by hand. It successfully suggested a range of other papers.

However, serious problems were encountered when attempting to use ScholarGPT to summarise papers. The summaries were found to have significant numbers of hallucinations, especially in the miscategorisations of themes. At least once, ScholarGPT inserted a reference to a nonexistent paper.

Once it became clear that ScholarGPT was miscategorising papers in the bibliography, the literature review was re-conducted using traditional means so that a detailed comparison could be made. Our comparison of theme categorisation is presented in Table \ref{scholargptcategorisations}.

ScholarGPT seemingly managed to assign roughly the same number of papers to themes as the human experimenter (it actually found one more than the human), but only 78\% (40 out of 52 total) of those themes were correctly assigned. 22\% (12 out of 40) of the themes identified by ScholarGPT were found to be incorrectly assigned.

\begin{table}[htp]
\caption{A Comparison of Human vs. ScholarGPT Theme Categorisations}
\begin{center}
\begin{tabular}{ | p{4cm} || p{2cm} | p{2cm} | p{2cm} |  }
 \hline
 Overall Theme & Assigned by Human & ScholarGPT Correctly Assigned & ScholarGPT Incorrectly Assigned \\
 \hline\hline
Applications of Web3 x AI & 7 & 7 & 5 \\ 
 \hline
 Cybersecurity & 3 & 2 & 1 \\  
 \hline
 Cyber Education & 1 & 1 & - \\  
 \hline
 Payment Security & 2 & 2 & - \\  
 \hline
 Defining Web3 x AI & 6 & 4 & - \\  
 \hline
 Software Auditing & 3 & 2 & - \\  
 \hline
 Sustainability & 4 & - & - \\  
 \hline
 Transaction Fraud Detection & 3 & 3 & 2 \\  
 \hline
 Machine Learning & 4 & 4 & - \\  
 \hline
 Standardization & 1 & - & 1 \\  
 \hline
 Transparent AI & 1 & 1 & - \\  
 \hline
 Internet of Things & 3 & 2 & - \\  
 \hline
 FinTech & 1 & 1 & 2 \\  
 \hline
 Theory of Mind & 2 & 2 & - \\  
 \hline
 Turing Test & 2 & 2 & - \\  
 \hline
 Copyright & 2 & 2 & 1 \\  
 \hline
 NFTs & 6 & 5 & - \\  
 \hline
 \hline
 \emph{Subtotals} & 51 & 40 & 12 \\
 \hline
\end{tabular}
\end{center}
\label{scholargptcategorisations}
\end{table}%

An attempt was also made to have ScholarGPT identify suggested future work in the bibliography and to categorise it via themes. The results are shown in Table \ref{scholargptfuturework}.

It should be noted that the ``Missing or incomplete themes'' Future Work Theme in Table \ref{scholargptfuturework} refers to authors who believe that we have not yet fully categorised the ways in which Web3 x AI integrations may occur.

ScholarGPT performed worse on the future work analysis than it did in overall theme assignment. It only managed to identify one third as many themes in the future work material as the human experimenter, with 40\% (4 out of 10) of the suggested themes being incorrectly assigned.

We conclude by suggesting that the relatively poor performance in identifying themes is much less important than the hallucinations that led to incorrect theme assignment. We might be tempted to further suggest that the hallucinations that are so critical to summarisation tasks in autoregressive (decoder-only) LLMs, such as ScholarGPT make the architecture itself a poor choice for tasks such as scholarly summaries. That is because incorrect or misleading summaries or theme assignments can easily lead less careful researchers into believing things that are not represented in the literature.


\begin{table}[htp]
\caption{A Comparison of Human vs. ScholarGPT Future Work Categorisations}
\begin{center}
\begin{tabular}{ | p{4cm} || p{2cm} | p{2cm} | p{2cm} |  }
 \hline
 Future Work Theme & Assigned by Human & ScholarGPT Correctly Assigned & ScholarGPT Incorrectly Assigned \\
 \hline\hline
 ``Singleton'' Web3 x AI & 3 & - & - \\ 
 \hline
 AI helping DAOs & 1 & - & - \\ 
 \hline
 AI helping software auditing & 5 & 1 & - \\ 
 \hline
 AI-based consensus & 1 & - & - \\ 
 \hline
 Quantum crypto protocols & 1 & - & 1 \\ 
 \hline
 Federated AI learning & 2 & - & - \\ 
 \hline
 Quantum/AI integration for DLT security & 1 & - & 1 \\ 
 \hline
 Missing or incomplete themes & 1 & - & - \\ 
 \hline
 Scalability & 1 & 1 & 1 \\ 
 \hline
 Transparent AI training & 3 & 1 & - \\ 
 \hline
 Web3-based AI marketplaces & 2 & - & - \\ 
 \hline
 Regulatory compliance \& ethical considerations & 6 & 2 & 1 \\ 
 \hline
 Economic impacts \& ownership & 4 & 1 & - \\ 
 \hline
 \hline
 \emph{Subtotals} & 31 & 6 & 4 \\
 \hline
\end{tabular}
\end{center}
\label{scholargptfuturework}
\end{table}%

